On the Transformations across Reward Model, Parameter Update, and In-Context Prompt

Despite the general capabilities of pre-trained large language models (LLMs), they still need further adaptation to better serve practical applications. In this paper, we demonstrate the interchangeability of three popular and distinct adaptation tools: parameter updating, reward modeling, and in-context prompting. This interchangeability establishes a triangular framework with six transformation directions, each of which facilitates a variety of applications. Our work offers a holistic view that unifies numerous existing studies and suggests potential research directions. We envision our work as a useful roadmap for future research on LLMs.

==> draft_conversion1.tex <==

Consider a reward model, denoted as $r(x, y)$, which assigns a scalar value to any pair of input $x$ and output $y$, serving as an indicator of the quality of $y$ in relation to $x$.
There is an initial language model $\pi_0$ that defines the conditional probability $\pi_0(y|x)$ of $y$ given $x$. Our objective is to update the model from $\pi_0$ to $\pi$ such that it maximizes the expected reward value from $r(x, y)$. In the meanwhile, we want to keep $\pi$ close to $\pi_0$ to prevent over-fitting or catastrophic forgetting \citep{ouyang2022training}. This optimization problem can be formalized as follows:
\begin{equation}
\max _{\pi} \mathbb{E}_{x\sim \mathcal{D}, y\sim \mathcal{\pi}(y|x)}\big[r_\phi(x, y)\big] - \beta \mathbb{D}_{\text{KL}}\big[\pi(y |x) || \pi_0(y | x) \big],
\label{maximize_reward}
\end{equation}
where the input $x$ is sampled from an empirical distribution $\mathcal{D}$ and $\beta$ is a hyper-parameter that controls the strength of regularization term, i.e., the KL distance between $\pi$ and $\pi_0$.

We can consider the above process as a transformation from a reward model to a parameter update. Specifically, we want to distill the preference knowledge previously captured by $r(x, y)$ into the parameter update from $\pi_0$ to $\pi$. Following \citet{rafailov2023direct} and \citet{mitchell2024an}, this can be further elucidated by writing down the optimal solution $\pi^*$ to Eq. \ref{maximize_reward} analytically.
\begin{equation}
  \pi^*(y|x) = \frac{1}{Z(x)} \pi_{0}(y|x) \exp(\frac{1}{\beta} r(x, y)),
\label{optimal_solution}
\end{equation}
where ${Z(x)}$ is the partition function. Obviously, directly computing the RHS of Eq. \ref{optimal_solution} is infeasible. In practice, this optimization process is often accomplished by reinforcement learning algorithms such as proximal policy optimization (PPO) \citep{schulman2017proximal,ouyang2022training}.
\paragraph{Applications} 
\cd{by Tingchen}




% first part: traditional RLHF with explicit reward model; 
A typical application of the transformation is aligning large language models with human-desired criteria or preferences \citep{ouyang2022training}.
Existing works either directly use human-annotated preference data or learn a parametric reward model as a proxy of humans to update an initial language model $\pi_0$ to an aligned one $\pi$, according to Eq~\ref{optimal_solution}. For instance, \citet{ouyang2022training} employ PPO~\citep{schulman2017proximal} to convert the pre-trained language model into an instruction follower. Since PPO is notorious for its complexity and instability, \citet{noukhovitch2023language} smooth the parameter updating by periodically resetting the $\pi$ to the exponentially moving average of the initial language model $\pi_0$ and \citet{li2023remax} substitute the complex PPO algorithm with REINFORCE~\citep{williams2004simple} to simplify the optimization process. 

% second part: implicit reward model 
As the conventional RLHF procedure is complicated and unstable in implementation, DPO~\citep{rafailov2023direct} has been proposed to solve the RLHF problem with a classification loss, bypassing explicit reward modeling and reinforcement learning. To be more specific, instead of materializing reward model explicitly on pairwise preference data, the language model itself acts as a secret reward model~\citep{rafailov2023direct} to construct implicit rewards: 
\begin{equation}
\begin{aligned}
&r^+ = \beta \log \pi (y_w | x) - \beta \log \pi_{0} (y_w | x), \\
&r^- = \beta \log \pi (y_l | x) - \beta \log \pi_{0} (y_l | x),
\end{aligned}
\end{equation}
and update the language model parameter to widen the margin between them:
\begin{equation}
\mathcal{L}_{{{\rm DPO}}} = - \mathbb{E}_{(x,y_w,y_l) \sim \mathcal{D}} \log {\rm sigmoid} (r^+ - r^-).
\end{equation}%% add more work for DPO variant
Following this direction, \citet{azar2023general} delve deeper into the behavior of DPO and identify its potential pitfall of overfitting caused by the implicit reward model. To deal with the issue, they propose an alternative IPO loss:
\begin{equation}
    \mathcal{L}_{{\rm{IPO}}} = \mathbb{E}_{(x, y_w, y_l)\sim \mathcal{D}} \left( r^+-r^- - \frac{\tau^{-1}}{2} \right)^2,  
\end{equation}
where $\tau$ is a real positive regularization parameter to train the language model until a desired improvement in implicit reward model is met.

% the third part: reward model with more than pairwise preference data. this is a little off-topic since it discusses the specific form of reward model. 
Despite its effectiveness and simplicity, DPO and IPO are specially tailored for pairwise preference data, overlooking other formats of human preference. On one hand, considering the cost of collecting pairwise data, KTO~\citep{ethayarajh2024kto} opts for maximizing the utility of language model generation from prospect theory and only requires a binary signal of whether an output is desirable or undesirable. On the other hand, to adapt the framework to preference data with $n$-length preference ranking, an intuitive idea is to keep the best one and a random one from the remaining responses to construct pairwise preference data~\citep{tunstall2023zephyr}, which fails to fully utilize the preference information. Alternatively, preference rank optimization~\citep{song2023preference} equips LLMs with multi-positional and multi-dimensional contrasts among responses by constructing multiple rewards:  
\begin{equation}
    r_i = \log \pi (y_i | x), \quad i=1,2,\ldots,n,
\end{equation}
where $y_i$ is the $i$-th response in the preference ranking. The language model is thereby optimized by the following objective:
\begin{equation}
    \mathcal{L}_{{\rm{PRO}}} = - \mathbb{E}_{(x,y_1,y_2,\ldots,y_n)\sim \mathcal{D}} \log \prod_{k=1}^{n-1}  \frac{\exp (r_k) }{ \sum_{i=k}^n \exp (r_i) }
\end{equation}
In a similar vein, \citet{chen2024noise} employ noise contrastive estimation to achieve human preference alignment on $n$-length preference ranking data.


In summary, in RLHF and its variants, the reward model acts as a proxy for human preference. Depending on the formats of collected human preference data (e.g., pairwise data~\citealp{bai2022training}, score-based data~\citealp{cui2023ultrafeedback}, or $n$-length rank~\citealp{song2023preference}), the specific form of the reward model varies significantly. Therefore, various techniques have been developed to update the language model parameter~\citep{schulman2017proximal,rafailov2023direct,ethayarajh2024kto}, adapting to different forms of human preferences and reward models.  



% the side note: implicit parameter update. 
Apart from directly inducing a concrete aligned language model $\pi$ with a reward model $r(x,y)$, a concurrent line of works attempts to bypass the parameter updating of $\pi_0$ in the weight space but interferes with the predicted logits of $\pi_0$ at output space to guide it towards the direction of LLM alignment. For example, \citet{khanov2024alignment,zhu2024proxy} adjust the predicted logits at every inference step by incorporating the reward on accepting each token as a continuation of the current prompt and generation. Furthermore, since a reward model is not intended to rate partially finished sentences, \citet{Huang2024deal} propose to generate continuations up to a certain lookahead length before evaluating the utility of each with a reward model. 

